Low Rank Learning for Offline Query Optimization

Recent deployments of learned query optimizers use expensive neural networks and ad-hoc search policies. To address these issues, we introduce \textsc{LimeQO}, a framework for offline query optimization leveraging low-rank learning to efficiently explore alternative query plans with minimal resource usage. By modeling the workload as a partially observed, low-rank matrix, we predict unobserved query plan latencies using purely linear methods, significantly reducing computational overhead compared to neural networks. We formalize offline exploration as an active learning problem, and present simple heuristics that reduces a 3-hour workload to 1.5 hours after just 1.5 hours of exploration. Additionally, we propose a transductive Tree Convolutional Neural Network (TCNN) that, despite higher computational costs, achieves the same workload reduction with only 0.5 hours of exploration. Unlike previous approaches that place expensive neural networks directly in the query processing ``hot'' path, our approach offers a low-overhead solution and a no-regressions guarantee, all without making assumptions about the underlying DBMS. The code is available in \href{https://github.com/zixy17/LimeQO}{https://github.com/zixy17/LimeQO}.

==> online_technique.tex <==
\section{Online Mode}
\label{sec:online-mode}

\rcm{Here, we present LimeQO's online mode, which, unlike the offline mode, XXX. While prior LQOs must deal with query regressions, LimeQO's restriction to repetitive queries means that our online mode can \emph{guarantee} improved tail performance compared to a baseline optimizer, and also bound the maximum possible regression for any single query. Under certain circumstances, LimeQO can even guarantee strictly better workload-level performance}

\subsection{Problem definition}

\rcm{Describe the setting, where now we process queries in an online fashion. When a new unique query arrives, we also use the default/baseline optimizer, and only potentially change QPs on the 2nd execution. This is a big restriction of scope compared to prior work, but this allows us to make performance guarantees}

\sparagraph{Bounding tail performance compared to a baseline optimizer} \rcm{Define what it means to bound tail performance compared to PG -- we can promise that limeqo will always decrease tail latency}

\sparagraph{Bounding regressions on individual queries} \rcm{workload level stats aren't enough, also need promises about each individual query, limeqo can promise that no query's performance will ever be worse than Kq seconds more than the default optimizer's performance, for a user-set K}

\subsection{Ensuring performance improvements}

\sparagraph{Workload-level tail latency} \rcm{surprisingly simple technique: keep track of how much headroom we have for a particular query, run an alternative plan with a timeout of that amount of headroom, if it fails, execute the original plan}

\sparagraph{Maximum query-level regression} \rcm{similar to above: given a Kq, see how much time we have to test a new query and do so if we can}

\sparagraph{Combining workload-level and query-level guarantees} \rcm{just take the min of the headroom from above}


